Globally Convergent Multilevel Training of Deep Residual Networks

We propose a globally convergent multilevel training method for deep residual networks (ResNets). The devised method can be seen as a novel variant of the recursive multilevel trust-region (RMTR) method, which operates in hybrid (stochastic-deterministic) settings by adaptively adjusting mini-batch sizes during the training. The multilevel hierarchy and the transfer operators are constructed by exploiting a dynamical system's viewpoint, which interprets forward propagation through the ResNet as a forward Euler discretization of an initial value problem. In contrast to traditional training approaches, our novel RMTR method also incorporates curvature information on all levels of the multilevel hierarchy by means of the limited-memory SR1 method. The overall performance and the convergence properties of our multilevel training method are numerically investigated using examples from the field of classification and regression.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
%\headers{Globally Convergent Multilevel Training of ResNets}{D. Doe, P. T. Frank, and J. E. Smith}
\headers{Globally Convergent Multilevel Training Of ResNets}{A. Kopani\v{c}\'akov\'a, R. Krause}


% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{An Example Article\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}
\title{Globally Convergent Multilevel Training of Deep Residual Networks\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Swiss National Science Foundation (SNF) under the project ML$^2$ (grant no.~197041) and by Platform for Advanced Scientific Computing (PASC) under the project EXATRAIN.}}}


% Authors: full names plus addresses.
\author{Alena Kopani\v{c}\'akov\'a \thanks{Euler Institute, Universit{\`a} della Svizzera italiana
  (\email{alena.kopanicakova@usi.ch}, \url{http://usi.to/r8u}).}
%\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
%  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Rolf Krause\footnotemark[2]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc}
\usepackage{caption}
\usepackage{algorithm,algpseudocode}
\usepackage{graphicx,url}
\usepackage{amsmath,amssymb,amsopn}
\usepackage{tabularx}
\usepackage{color}
\usepackage{calc}
\usepackage{caption}
\usepackage{longtable}
\usepackage{multirow}
\usepackage{mathrsfs}
\usepackage{array}
\usepackage{hyperref}
\usepackage{tikz}
\usepackage{booktabs}
\usepackage{pgfplotstable}
\usepackage{pgfplots}
\usepackage[outline]{contour}
\usepackage[colorinlistoftodos,prependcaption]{todonotes}
\usepackage{calrsfs}
\usepackage{graphicx}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{matrix}
\usetikzlibrary{automata, external, shapes.geometric, fit}
\tikzexternalize[prefix=tikzpics/]

\pgfplotsset{compat=1.13}


%%%%%%%%%%%% vectors %%%%%%%%%%%%
\def \av{\vec{a}}
\def \bv{\vec{b}}
\def \cv{\vec{c}}
\def \dv{\vec{d}}
\def \ev{\vec{e}}
\def \fv{\vec{f}}
\def \gv{\vec{g}}
\def \hv{\vec{h}}
\def \iv{\vec{i}}
\def \jv{\vec{j}}
\def \kv{\vec{k}}
\def \lv{\vec{l}}
\def \mv{\vec{m}}
\def \nv{\vec{n}}
\def \ov{\vec{o}}
\def \pv{\vec{p}}
\def \rv{\vec{r}}
\def \sv{\vec{s}}
\def \tv{\vec{t}}
\def \uv{\vec{u}}
\def \vv{\vec{v}}
\def \wv{\vec{w}}
\def \xv{\vec{x}}
\def \yv{\vec{y}}
\def \zv{\vec{z}}
\def \thetav{\vec{\theta}}




%%%%%%%%%%%% vectors capital %%%%%%%%%%%%
\def \Av{\vec{A}}
\def \Bv{\vec{B}}
\def \Cv{\vec{C}}
\def \Dv{\vec{D}}
\def \Ev{\vec{E}}
\def \Fv{\vec{F}}
\def \Gv{\vec{G}}
\def \Hv{\vec{H}}
\def \Iv{\vec{I}}
\def \Jv{\vec{J}}
\def \Kv{\vec{K}}
\def \Lv{\vec{L}}
\def \Mv{\vec{M}}
\def \Nv{\vec{N}}
\def \Ov{\vec{O}}
\def \Pv{\vec{P}}
\def \Rv{\vec{R}}
\def \Sv{\vec{S}}
\def \Tv{\vec{T}}
\def \Uv{\vec{U}}
\def \Vv{\vec{V}}
\def \Wv{\vec{W}}
\def \Xv{\vec{X}}
\def \Yv{\vec{Y}}
\def \Zv{\vec{Z}}



%%%%%%%%%%%% matrices %%%%%%%%%%%%
\def \am{\mat{a}}
\def \bm{\mat{b}}
\def \cm{\mat{c}}
\def \dm{\mat{d}}
%\def \em{\mat{e}}
\def \fm{\mat{f}}
\def \gm{\mat{g}}
\def \hm{\mat{h}}
\def \im{\mat{i}}
\def \jm{\mat{j}}
\def \km{\mat{k}}
\def \lm{\mat{l}}
\def \mm{\mat{m}}
\def \nm{\mat{n}}
\def \om{\mat{o}}
%\def \pm{\mat{p}}
\def \rm{\mat{r}}
%\def \sm{\mat{s}}
\def \tm{\mat{t}}
\def \um{\mat{u}}
\def \vm{\mat{v}}
\def \wm{\mat{w}}
\def \xm{\mat{x}}
\def \ym{\mat{y}}
\def \zm{\mat{z}}



%%%%%%%%%%%% matrices capital %%%%%%%%%%%%
\def \Am{\mat{A}}
\def \Bm{\mat{B}}
\def \Cm{\mat{C}}
\def \Dm{\mat{D}}
\def \Em{\mat{E}}
\def \Fm{\mat{F}}
\def \Gm{\mat{G}}
\def \Hm{\mat{H}}
\def \Im{\mat{I}}
\def \Jm{\mat{J}}
\def \Km{\mat{K}}
\def \Lm{\mat{L}}
\def \Mm{\mat{M}}
\def \Nm{\mat{N}}
\def \Om{\mat{O}}
\def \Qm{\mat{Q}}
\def \Pm{\mat{P}}
\def \Rm{\mat{R}}
\def \Sm{\mat{S}}
\def \Tm{\mat{T}}
\def \Um{\mat{U}}
\def \Vm{\mat{V}}
\def \Wm{\mat{W}}
\def \Xm{\mat{X}}
\def \Ym{\mat{Y}}
\def \Zm{\mat{Z}}



%%%%%%%%%%%% mathbb %%%%%%%%%%%%
\def \R{\mathbb{R}}			% real numbers
\def \N {\mathbb{N}}			% nat. numbers
\def \E {\mathbb{E}}			% nat. numbers


%%%%%%%%%%%% pazocal %%%%%%%%%%%%
\def \D{\pazocal{D}}			% Hessian approximation
\def \H{\pazocal{H}}			% hypothesis function
\def \L{\pazocal{L}}			% 
\def \Reg{\pazocal{R}} 		% regularization term
\def \D{\pazocal{D}} 			% dataset
\def \F{\pazocal{F}} 





\DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}
%\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}
%\DeclareMathAlphabet{\mathsfbfit}{\encodingdefault}{\sfdefault}{bx}{sl}
%\DeclareMathAlphabet{\mathbfit}{\encodingdefault}{\rmdefault}{b}{it}
%\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}

\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\tens}[1]{\mathsfbfit{#1}}
\newcommand{\fourtens}[1]{\mathds{#1}}
\newcommand{\greektens}[1]{\boldsymbol{#1}}
\newcommand{\tenscomponent}[1]{\mathsfit{#1}}


% -------------- algo commands  -------------
\algnewcommand\algorithmiconput{\textbf{Constants:}}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand{\algorithmicgoto}{\textbf{go to}}%


\algnewcommand\Constants{\item[\algorithmiconput]}
\algnewcommand\Input{\item[\algorithmicinput]}%
\algnewcommand\Output{\item[\algorithmicoutput]}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%


%\theoremstyle{definition}
%\newtheorem{example}{Example}[section]
%\newtheorem*{assumption}{Assumption}



%%%%%%%%%%%%%% colors %%%%%%%%%%%%%%
\definecolor{myblack}{RGB}{53, 53, 53}
\definecolor{myblue}{RGB}{40, 75, 99}
\definecolor{myred}{RGB}{192, 50, 33}
\definecolor{myyellow}{RGB}{255, 166, 48}
\definecolor{mywhite}{RGB}{240, 237, 238}
\definecolor{mygreen}{RGB}{0, 102, 0}


\definecolor{green1}{RGB}{9, 82, 86}
\definecolor{green2}{RGB}{8, 127, 140}
\definecolor{green3}{RGB}{6, 167, 125}
\definecolor{green4}{RGB}{79, 109, 122}
\definecolor{green5}{RGB}{192, 214, 223}
\definecolor{violet}{RGB}{26,69,131}

\definecolor{checkgreen}{rgb}{0,0.6,0}
\definecolor{phase1}{rgb}{0.008,0.655,1.000}
\definecolor{phase2}{rgb}{0.016,0.75,0.700}
\definecolor{phase3}{rgb}{0.929,0.35,0.700}
\definecolor{icsyellow}{cmyk}{0.00,0.11,0.53,0.00}




\definecolor{blackmy}{RGB}{38, 70, 83}

\definecolor{bluemy}{RGB}{39, 125, 161}
\definecolor{greenmy}{RGB}{42, 167, 143}
\definecolor{yellowmy}{RGB}{233, 196, 106}
\definecolor{brownmy}{RGB}{244, 162, 97}
%\definecolor{brownmy}{RGB}{249, 132, 74}
%\definecolor{orangemy}{RGB}{231, 111, 81}
\definecolor{redmy}{RGB}{249, 65, 68}






